Adversarial Machine Learning Threats to Spacecraft

Spacecraft are among the earliest autonomous systems. Their ability to function without a human in the loop have afforded some of humanity's grandest achievements. As reliance on autonomy grows, space vehicles will become increasingly vulnerable to attacks designed to disrupt autonomous processes-especially probabilistic ones based on machine learning. This paper aims to elucidate and demonstrate the threats that adversarial machine learning (AML) capabilities pose to spacecraft. First, an AML threat taxonomy for spacecraft is introduced. Next, we demonstrate the execution of AML attacks against spacecraft through experimental simulations using NASA's Core Flight System (cFS) and NASA's On-board Artificial Intelligence Research (OnAIR) Platform. Our findings highlight the imperative for incorporating AML-focused security measures in spacecraft that engage autonomy.

==> notes.tex <==
Autonomous landing on the Moon is a complex operation where precision and safety are paramount. Various models and filters, including those discussed, can be crucial in ensuring a successful landing. Here’s how a linear regression model and a Kalman Filter might be used in different stages of a lunar landing mission:

1. Descent Trajectory Prediction
Linear Regression Model:

Purpose: Before the descent begins, a linear regression model can predict the optimal descent trajectory based on historical data from previous missions and simulations. This model could analyze how changes in spacecraft orientation and velocity at different altitudes have impacted the descent path and landing accuracy in past missions.
Usage: By understanding these relationships, mission planners can program initial descent parameters that optimize fuel use, minimize landing errors, and account for expected lunar surface conditions.
2. Real-Time Navigation and Adjustment
Kalman Filter:

Purpose: During the descent, a Kalman Filter becomes essential. It continuously estimates the current state of the spacecraft (position, velocity, and acceleration) using real-time data from onboard sensors like accelerometers, gyroscopes, altimeters, and radar.
Usage: As the spacecraft descends, the Kalman Filter adjusts the predicted state by filtering out noise and inaccuracies from sensor readings. This real-time state estimation allows the spacecraft to make precise adjustments to its thrusters and control surfaces, ensuring it follows the optimal path to the landing site.
3. Approach and Touchdown
Combination of Models:

Sensor Fusion: As the spacecraft approaches the surface, data from visual, radar, and laser altimeters are integrated using sensor fusion techniques, potentially managed by a Kalman Filter, to accurately determine the distance to the lunar surface and identify obstacles.
Final Adjustments: The linear regression model could additionally provide predictions on how final maneuvers (like last-minute course corrections and hover operations) will affect the landing dynamics, based on the current velocity and angular orientation. This helps in fine-tuning the descent without overcorrecting, which is critical in the low-gravity, no-atmosphere environment of the Moon.
4. Hazard Avoidance
Real-Time Decision Making: Both models contribute to an autonomous hazard detection and avoidance system. As the Kalman Filter updates the spacecraft's state, the regression model can predict potential hazards based on the current trajectory and surface conditions (like

\textbf{USE THIS FOR EXPLANATION: 
}
In a real-time spacecraft operation, particularly during critical maneuvers like lunar landing or orbital insertion, a linear regression model like the one described could be used to enhance predictive accuracy and operational efficiency. Here’s an example scenario illustrating how this might work during a lunar landing:

Context: Lunar Landing Maneuver
As a spacecraft approaches the Moon's surface, precise control over its descent trajectory, velocity, and attitude (orientation) is crucial. Anomalies in predicted versus actual parameters can result in mission failure. Using a linear regression model trained on past mission data or simulations, the control system can refine its predictions and adjustments in real-time.

Real-Time Application of the Linear Regression Model
Pre-Descent Calibration:
Before initiating the descent, the linear regression model processes the last set of telemetry data to predict the initial descent behavior based on known variables like altitude, velocity, and angular orientation.
This model has been trained to understand how certain inputs correlate with changes in velocity and angle, helping predict how the spacecraft will behave once the descent starts.
Descent Phase Integration:
As the spacecraft descends, its sensors continuously feed new data about its velocity and angle changes back to the onboard computer.
The linear regression model updates its predictions in real-time, recalculating expected velocity and angular changes based on the most recent data.
Feedback to Control Systems:
The predictions from the linear regression model are used to adjust the control commands. For instance, if the model predicts a faster velocity decrease than desired, the descent engine's thrust might be modulated to correct this.
This predictive feedback loop helps maintain an optimal descent profile, ensuring the spacecraft lands at the designated site with minimal fuel consumption and risk.
Anomaly Detection and Correction:
The model can also serve as a benchmark for expected vs. actual parameters. If real-time data significantly deviates from model predictions, it can trigger a diagnostic or alert the mission control to potential issues.
Quick corrective actions can be taken, either automatically by the onboard systems or manually by ground control, based on the severity and nature of the deviation.
Post-Landing Analysis:
After landing, the data and the model's performance are analyzed to improve the accuracy of the model for future missions. This could involve retraining the model with new data gathered during the descent to refine its predictive accuracy.
Conclusion
In this scenario, the linear regression model acts as a critical component of the spacecraft’s GNC system by providing predictive insights that help fine-tune control algorithms in real time. It enhances the spacecraft's ability to adapt to dynamic conditions, improves safety and efficiency, and helps ensure that the landing process adheres to planned parameters. This application of machine learning models like linear regression in spacecraft operations exemplifies the integration of advanced analytics into traditional aerospace engineering.



\textbf{APPENDIX} 

import pandas as pd  # Data handling, needed for loading historical or pre-mission data for model training
from sklearn.model_selection import train_test_split  # Splitting data into training and testing sets for model validation
from sklearn.linear_model import SGDRegressor  # The regression model to predict velocity and angle changes
from sklearn.metrics import mean_squared_error  # Evaluates model accuracy to ensure reliable predictions
from sklearn.preprocessing import StandardScaler  # Standardizing input features to improve model performance
import os  # Handling file paths for loading data

data_directory = '/home/aal/cFS/build/exe/cpu1/OnAIR/'
os.chdir(data_directory)  # Changing to the directory with telemetry data, crucial for data access

# Loading and preparing telemetry data which will be used to train the model before real-time deployment
try:
    df = pd.read_csv('dlc.csv', delimiter='\t')  # Assuming tab-delimited, real telemetry data from simulations or past missions
except FileNotFoundError:
    print("Error: File 'dlc.csv' not found. Please check the file path.")
    exit(1)

df.columns = df.columns.str.strip()  # Clean up column names to ensure accurate feature selection

print("Columns in the DataFrame:", df.columns)  # Verify data structure, crucial for debugging and validation

# Specify columns relevant to GNC tasks such as velocity and angular changes
selected_columns = [
    'DATA_DELTA_VEL[2]',
    'DATA_DELTA_VEL[3]',
    'DATA_DELTA_ANGLE[1]',
    'DATA_DELTA_ANGLE[2]',
    'DATA_DELTA_ANGLE[3]'
]

# Ensuring all necessary data columns are present for accurate model training
missing_columns = [col for col in selected_columns if col not in df.columns]
if missing_columns:
    print(f"Error: The following columns are missing in the DataFrame: {missing_columns}")
    exit(1)

# Set up data for model input (features) and output (target) for prediction
X = df[selected_columns]
y = df['DATA_DELTA_VEL[1]']  # Example target variable, a specific velocity change

# Normalizing data to ensure consistent scale, crucial for accurate predictive modeling
scaler = StandardScaler()
X_scaled = scaler.fit_transform(X)

# Splitting the data to train the model and then validate it, ensuring it performs well under test conditions
X_train, X_test, y_train, y_test = train_test_split(X_scaled, y, test_size=0.2, random_state=42)

# Testing various learning rates to optimize model performance, essential for real-time application
learning_rates = [0.001, 0.01, 0.1, 0.5]
for learning_rate in learning_rates:
    model = SGDRegressor(learning_rate='constant', eta0=learning_rate, random_state=42)
    model.fit(X_train, y_train)  # Training the model with training dataset

    # Output learning rates and coefficients to monitor how well the model is learning and to adjust if necessary
    print(f"\nLearning Rate: {learning_rate}")
    print("Coefficients:", model.coef_)

    # Use the test set to predict and calculate mean squared error for model evaluation
    y_pred = model.predict(X_test)
    mse = mean_squared_error(y_test, y_pred)
    print(f'The mean squared error of the model is {mse:.2f} with a learning rate of {learning_rate}.')



---
